Exploring Multi-dimensional Data via Subset Embedding

Multi-dimensional data exploration is a classic research topic in visualization. Most existing approaches are designed for identifying record patterns in dimensional space or subspace. In this paper, we propose a visual analytics approach to exploring subset patterns. The core of the approach is a subset embedding network (SEN) that represents a group of subsets as uniformly-formatted embeddings. We implement the SEN as multiple subnets with separate loss functions. The design enables to handle arbitrary subsets and capture the similarity of subsets on single features, thus achieving accurate pattern exploration, which in most cases is searching for subsets having similar values on few features. Moreover, each subnet is a fully-connected neural network with one hidden layer. The simple structure brings high training efficiency. We integrate the SEN into a visualization system that achieves a 3-step workflow. Specifically, analysts (1) partition the given dataset into subsets, (2) select portions in a projected latent space created using the SEN, and (3) determine the existence of patterns within selected subsets. Generally, the system combines visualizations, interactions, automatic methods, and quantitative measures to balance the exploration flexibility and operation efficiency, and improve the interpretability and faithfulness of the identified patterns. Case studies and quantitative experiments on multiple open datasets demonstrate the general applicability and effectiveness of our approach.

==> contents/ExpertFeedback.tex <==
\section{Expert Feedback}

We established a remote contact with a data analysis expert to collect his comments and suggestions on our approach. The expert works in the data analysis department of a famous IT company. He has led many projects concerning public security data analysis. 

We first introduced the SEN and demonstrated how to use the visualization system to find patterns on the Chicago crime dataset. We encouraged the expert to ask any questions and make sure he can understand the general idea and the usage of the visualization system. We then had a free discussion for about 20 minutes. Generally, the expert’s feedback was very encouraging while pointing at some aspects requiring improvement, as follows:

The overall feedback of the expert is positive. He said: “I never thought data can be analyzed at the subset level, which can find more interesting patterns.” He highly praised the SEN. The multi-subnet structure, the loss functions, and the high training efficiency impressed him much. The expert thought the visual design can be easily understood. He believed using a tree to manage the exploration process is intuitive. He also confirmed the effectiveness of the querying and clustering functions that save much time in searching for subsets involving patterns in the projection.

The expert pointed out that users of our system should have much expertise in data analysis. He said: “Many critical operations of the visualization system are conducted manually, which may affect its popularity among ordinary users.” He suggested to further simplify the interface and interactions for these users. The expert also expressed a cooperation desire to apply the tool in his projects. He suggested us to add more data management functions, such as data preprocessing, subset feature customization, etc., and release a business version as soon as possible.


